Stochastic Linear Optimization with Adversarial Corruption

We extend the model of stochastic bandits with adversarial corruption (Lykouriset al., 2018) to the stochastic linear optimization problem (Dani et al., 2008). Our algorithm is agnostic to the amount of corruption chosen by the adaptive adversary. The regret of the algorithm only increases linearly in the amount of corruption. Our algorithm involves using L\"owner-John's ellipsoid for exploration and dividing time horizon into epochs with exponentially increasing size to limit the influence of corruption.

==> Figure/random-pricing-approx-opt.tex <==
\begin{tikzpicture}[scale = 0.5]


% \fill[gray!40!white] (0, 0) -- (5, 5) -- (5, 7.5) -- (0,7.5);

\draw (-0.2,0) -- (14.2, 0);
\draw (0, -0.2) -- (0, 8.2);
\draw (14, 0.2) -- (14, -0.2);
\draw (-0.2, 8) -- (0.2, 8);


\begin{scope}[very thick]
\draw plot [smooth, tension=0.6] coordinates { (0,0) (1,4) (5,5.5) (10,5)};
\draw [name path = A] plot [smooth, tension=0.6] coordinates { (10,5) (12,3.5) (14,0)};
\draw [name path = B] (0, 0) -- (10, 5);
\tikzfillbetween[of=A and B]{gray!40!white};
\fill[gray!40!white] (0, 0) -- (10, 5) -- (14, 0) -- (0,0);
\draw [gray!40!white] (10, 5) -- (14, 0);
\draw plot [smooth, tension=0.6] coordinates { (10,5) (12,3.5) (14,0)};
\draw (0, 0) -- (12, 6);

% \draw (5, 5) -- (5, 7.5);
% \draw (5, 7.5) -- (10,7.5);

%\draw [dashed] (0, 0) -- (10, 10);
\end{scope}

% \draw [name path = D, dashed]
% (6.3, 7) -- (10, 7);


\draw (0, -0.8) node {$0$};
\draw (14, -0.8) node {$1$};

\draw (-0.6, 0) node {$0$};
\draw (-0.6, 8) node {$1$};


\end{tikzpicture}

==> Paper/exploration.tex <==
\section{Exploration by Coordinate}

First, we give a simple algorithm based on a strong assumption of the decision set $\xSet$.
Suppose that there exists a set of points $\exploreSet^+ \cup \exploreSet^- \subseteq \xSet$ such that these points make up 
$\dimension$ pairs $(\explore^+_j,\explore^-_j)$ 
with $\explore^+_j \in \exploreSet^+$ and $\explore^-_j \in \exploreSet^-$. 
And we have $\explore^+_j-\explore^-_j = \explore_j$ is the standard basis vector in $\reals^\dimension$.
For instance, if $\xSet$ is the simplex with dimension $\dimension$, 
then $\xSet$ satisfies the assumption. 

The detail of our algorithm is shown in~\Cref{alg:explobycoor}.   
Intuitively, our algorithm proceeds in epochs with exponentially increasing length $\totalnum_\epoch$. 
In each epoch $\epoch$, it randomly chooses one of the two operations. 
With probability $\gamma_{\epoch-1}$, 
it uniformly samples one point from the explore set $\exploreSet^+ \cup \exploreSet^-$. 
Otherwise, it chooses the best vector $\context^{(\epoch-1)}_*$ 
according to the empirical estimation $\empirical^{\epoch-1}$ in the previous epoch. 

\input{Paper/algorithm.tex}

% \begin{lemma}[\citet{abbasi2011improved}]
% \label{lem:martingale concentration}
% $\norm{S_t}_{\sumContext_t}^2 \leq $
% \end{lemma}

\begin{lemma}
\label{lem:estimate theta}
With probability at least $1-\confidence$, the estimation $\empirical^\epoch$ satisfies for all $j \in [\dimension]$,
\begin{align*}
    \abs{\empirical_j^{(\epoch)} - \hidden_j} \leq \frac{\empiricaldiff^{(\epoch-1)}}{32 \sqrt{\dimension}}+ \frac{2\corruption_\epoch}{\totalnum_\epoch}.
\end{align*}
\end{lemma}

\begin{proof}
For any $j \in [\dimension]$, let $\xi_{j,+}^t$ be an indicator 
that choose the action $\explore^+_j$ in round $t$. Let $\num_e^{(\epoch)}$ be the expected number of rounds to explore $\explore^+_j$.
Then, the average reward for $\explore^+_j$ in epoch $\epoch$ is 
\begin{align*}
    \reward^{(\epoch)}_{j,+} = \frac{1}{\num_e^{(\epoch)}} \sum_{t= \horizon_{m-1} + 1}^{\horizon_m} \xi_{j,+}^t\slr{\inner{\explore^+_j }{\hidden} + \noise_t + \corruptionf_t(\explore^+_j)}.
\end{align*}
Since the choice of action $\explore^+_j$ 
is independent of the reward, noise and corruption, 
taking the expectation over the randomness of  $\xi_{j,+}^t$, we have
\begin{align*}
    \expect{\reward^{\epoch}_{j,+}} = \inner{\explore^+_j}{\hidden} + \frac{1}{\totalnum_\epoch} \sum_{t= \horizon_{m-1} + 1}^{\horizon_m} \corruptionf_t(\explore^+_j).
\end{align*}
Using Chernoff-Hoeffding bounds in \Cref{lem:concentration}, 
we can get that for any deviation $\beta$, 
\begin{align*}
&\prob{\abs{\reward^{\epoch}_{j,+} 
- \expect{\reward^{\epoch}_{j,+}}} \geq \beta} \\
\leq &
\prob{\abs{\frac{1}{\num_e^{(\epoch)}} \sum_{t= \horizon_{m-1} + 1}^{\horizon_m} \xi_{j,+}^t \cdot \noise_t 
} 
\geq \frac{\beta}{2}} 
+ 
\prob{\abs{\frac{1}{\num_e^{(\epoch)}} \sum_{t= \horizon_{m-1} + 1}^{\horizon_m} \xi_{j,+}^t\slr{\inner{\explore^+_j }{\hidden} + \corruptionf_t(\explore^+_j)} 
- \expect{\reward^{\epoch}_{j,+}}} 
\geq \frac{\beta}{2}} \\
\leq &
2\exp\blr{-\frac{\beta^2 \num_e^{(\epoch)}}{8}} 
+ 2\exp\blr{-\frac{\beta^2 \slr{\num_e^{(\epoch)}}^2}
{\sfrac{2\corruption_\epoch \num_e^{(\epoch)}}{\totalnum_\epoch} 
+ \beta \num_e^{(\epoch)}}} \leq 4\exp\blr{-\frac{\beta^2 \num_e^{(\epoch)}}{8}}.
\end{align*}
Similarly,
\begin{align*}
\prob{\abs{\reward^{\epoch}_{j,-} - \expect{\reward^{\epoch}_{j,-}}} \geq \beta} 
\leq 
4\exp\blr{-\frac{\beta^2 \num_e^{(\epoch)}}{8}}.
\end{align*}
Thus, 
\begin{align*}
    &\prob{\abs{(\reward^{\epoch}_{j,+} - \reward^{\epoch}_{j,-}) -  (\expect{\reward^{\epoch}_{j,+}}- \expect{\reward^{\epoch}_{j,-}})} \geq \beta} \\
    &\leq \prob{\abs{\reward^{\epoch}_{j,+} - \expect{\reward^{\epoch}_{j,+}}} \geq \frac{\beta}{2}} + \prob{\abs{\reward^{\epoch}_{j,-} - \expect{\reward^{\epoch}_{j,-}}} \geq \frac{\beta}{2}} \\
    &\leq 8\exp\blr{-\frac{\beta^2 \num_e^{(\epoch)}}{32}}.
\end{align*}
We have  $\num_e^{(\epoch)} = \frac{1}{2\dimension} \parameter (\empiricaldiff^{(\epoch-1)})^{-2}$. 
Let $\epsilon = \confidence / (\dimension \log{\horizon})$ and $\beta = \sqrt{64 \log(8/\epsilon) / \num_e^{(\epoch)}}$. 
Since $\parameter = 2^{14}\dimension^2 \log(8/\epsilon)$, we can derive
\begin{align*}
    \prob{\abs{\empirical^{(\epoch)}_j - \hidden_j} \geq \frac{2\corruption_\epoch}{\totalnum_\epoch} + \frac{\empiricaldiff^{(\epoch-1)}}{32\sqrt{\dimension}}} \leq \frac{\confidence}{\dimension \log{\horizon}}.
\end{align*}
\end{proof}

Let $\event = \blr{\forall \epoch \in [\log{T}]: \norm{\empirical^{(\epoch)} - \hidden}_2 \leq \frac{2\sqrt{\dimension}\corruption_\epoch}{\totalnum_\epoch} + \frac{\empiricaldiff^{(\epoch-1)}}{32} }$ be the event that
the true hidden vector is in the confident set 
of the estimated hidden vector 
at any time $t$. 
By the~\cref{lem:estimate theta}, we can get

\begin{lemma}
\label{lem:confidence interval}
The event $\event$ happens with probability at least $1-\confidence$, i.e. $\prob{\event}\geq 1-\confidence$.
\end{lemma}

\begin{proof}
According to~\cref{lem:estimate theta}, using the union bound over all $\log{\horizon}$ epochs and $\dimension$ coordinates implies that with probability at least $1-\confidence$, for all epoch $\epoch$
\begin{align*}
    \norm{\empirical^{(\epoch)} - \hidden}_2 
    \leq \sqrt{d\slr{\frac{2\corruption_\epoch}{\totalnum_\epoch} 
    + \frac{\empiricaldiff^{(\epoch-1)}}{32\sqrt{\dimension}}}^2} 
    = \frac{2\sqrt{\dimension}\corruption_\epoch}{\totalnum_\epoch} 
    + \frac{\empiricaldiff^{(\epoch-1)}}{32} \triangleq \estimationdiff_\epoch.
\end{align*}
\end{proof}



